Conformal Correction for Efficiency May be at Odds with Entropy

Conformal prediction (CP) provides a comprehensive framework to produce statistically rigorous uncertainty sets for black-box machine learning models. To further improve the efficiency of CP, conformal correction is proposed to fine-tune or wrap the base model with an extra module using a conformal-aware inefficiency loss. In this work, we empirically and theoretically identify a trade-off between the CP efficiency and the entropy of model prediction. We then propose an entropy-constrained conformal correction method, exploring a better Pareto optimum between efficiency and entropy. Extensive experimental results on both computer vision and graph datasets demonstrate the efficacy of the proposed method. For instance, it can significantly improve the efficiency of state-of-the-art CP methods by up to 34.4%, given an entropy threshold.

==> tables/cv-alpha-2.tex <==
\begin{table*}[t]
    \centering
    \caption{The efficiency results of conformal correction methods on CV datasets when $\alpha=0.2$. The results are the average of five runs of pre-trained model, each with 100 runs of conformal splits on CV datasets. 
    The best results are in shadow.}
    \setlength{\tabcolsep}{2.9mm}{
      \begin{tabular}{lccccccc}
      \toprule
      \multirow{2}{*}{Dataset} & \multirow{2}{*}{Model} & \multicolumn{2}{c}{CP} & \multicolumn{2}{c}{ConfTr} & \multicolumn{2}{c}{CCN} \\
      \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}
       &  & Coverage & Efficiency & Coverage & Efficiency & Coverage & Efficiency \\
      \midrule
      \multirow{3}*{CIFAR10} & ResNet56 
      & $0.80{\scriptstyle\pm.00}$ 
      & $4.01{\scriptstyle\pm.04}$ 
      & $0.80{\scriptstyle\pm.00}$
      & $1.06{\scriptstyle\pm.01}$ 
      & $0.80{\scriptstyle\pm.00}$ 
      & \hl{$1.04{\scriptstyle\pm.01}$} \\
      & PreResNet110 
      & $0.80{\scriptstyle\pm.00}$ 
      & $4.22{\scriptstyle\pm.09}$ 
      & $0.80{\scriptstyle\pm.00}$
      & \hl{$1.01{\scriptstyle\pm.02}$}
      & $0.80{\scriptstyle\pm.00}$ 
      & $1.02{\scriptstyle\pm.01}$ \\
      & DenseNet100            
      & $0.80{\scriptstyle\pm.00}$ 
      & $4.20{\scriptstyle\pm.02}$
      & $0.80{\scriptstyle\pm.00}$  
      & $0.99{\scriptstyle\pm.00}$ 
      & $0.80{\scriptstyle\pm.00}$ 
      & \hl{$0.98{\scriptstyle\pm.00}$} \\
        \midrule
       \multirow{3}*{CIFAR100}& ResNet56 
       & $0.80{\scriptstyle\pm.00}$ 
       & $13.38{\scriptstyle\pm.36}$ 
       & $0.80{\scriptstyle\pm.00}$  
       & $6.17{\scriptstyle\pm.75}$ 
       & $0.80{\scriptstyle\pm.00}$ 
       & \hl{$2.93{\scriptstyle\pm.09}$} \\
       & PreResNet110 
       & $0.80{\scriptstyle\pm.00}$ 
       & $14.98{\scriptstyle\pm.24}$ 
       & $0.80{\scriptstyle\pm.00}$  
       & $4.72{\scriptstyle\pm.10}$ 
       & $0.80{\scriptstyle\pm.00}$ 
       & \hl{$4.25{\scriptstyle\pm.17}$} \\
       & DenseNet100 
       & $0.80{\scriptstyle\pm.00}$ 
       & $18.13{\scriptstyle\pm1.28}$ 
       & $0.80{\scriptstyle\pm.00}$  
       & $3.20{\scriptstyle\pm.09}$ 
       & $0.80{\scriptstyle\pm.00}$ 
       & \hl{$2.76{\scriptstyle\pm.16}$} \\
      \bottomrule
      \end{tabular}}
    \label{T:cv-alpha-2}
\end{table*}

==> tables/cv-entropy-1.tex <==
\begin{table*}[t]
    \centering
    \caption{The entropy results of conformal correction methods on CV datasets when $\alpha=0.1$. The results are the average of five runs of pre-trained model, each with 100 runs of conformal splits on CV datasets.}
    \setlength{\tabcolsep}{3.5mm}{
      \begin{tabular}{lcccc}
      \toprule
       {Dataset} & {Model} & {CP} & {ConfTr} & {CCN} \\
      \midrule
      \multirow{3}*{CIFAR10} & ResNet56 
      & $0.19{\scriptstyle\pm.01}$
      & $2.73{\scriptstyle\pm.40}$ 
      & $2.97{\scriptstyle\pm.10}$ \\
       & PreResNet110  
       & $0.17{\scriptstyle\pm.01}$ 
       & $2.79{\scriptstyle\pm.40}$ 
       & $2.99{\scriptstyle\pm.19}$ \\
        & DenseNet100  
        & $0.16{\scriptstyle\pm.00}$ 
        & $2.55{\scriptstyle\pm.58}$ 
        & $2.94{\scriptstyle\pm.50}$ \\
        \midrule
       \multirow{3}*{CIFAR100} 
        & ResNet56  
        & $0.62{\scriptstyle\pm.09}$
        & $2.93{\scriptstyle\pm.51}$ 
        & $4.26{\scriptstyle\pm.61}$ \\
        & PreResNet110 
        & $0.67{\scriptstyle\pm.03}$ 
        & $3.16{\scriptstyle\pm1.06}$ 
        & $4.52{\scriptstyle\pm.48}$ \\
        & DenseNet100 
        & $0.57{\scriptstyle\pm.02}$ 
        & $2.49{\scriptstyle\pm.40}$ 
        & $4.14{\scriptstyle\pm.48}$ \\
      \bottomrule
      \end{tabular}}
    \label{T:xxx}
\end{table*}

==> tables/cv-entropy-2.tex <==
\begin{table*}[t]
    \centering
    \caption{The entropy results of conformal correction methods on CV datasets when $\alpha=0.2$. The results are the average of five runs of pre-trained model, each with 100 runs of conformal splits on CV datasets.}
    \setlength{\tabcolsep}{3.5mm}{
      \begin{tabular}{lccccc}
      \toprule
       {Dataset} & {Model} & {CP} & {ConfTr} & {CCN} \\
      \midrule
      \multirow{3}*{CIFAR10} & ResNet56 & $0.19{\scriptstyle\pm.01}$ & $2.99{\scriptstyle\pm.00}$ & $2.98{\scriptstyle\pm.01}$ \\
       & PreResNet110  & $0.17{\scriptstyle\pm.01}$ & $2.94{\scriptstyle\pm.03}$ & $2.99{\scriptstyle\pm.01}$ \\
        & DenseNet100  & $0.16{\scriptstyle\pm.00}$ & $2.97{\scriptstyle\pm.02}$ & $2.99{\scriptstyle\pm.01}$ \\
        \midrule
       \multirow{3}*{CIFAR100}
        & ResNet56  
        & $0.64{\scriptstyle\pm.09}$ 
        & $1.73{\scriptstyle\pm.11}$ 
        & $2.93{\scriptstyle\pm.09}$ \\
        & PreResNet110 
        & $0.65{\scriptstyle\pm.03}$ 
        & $1.60{\scriptstyle\pm.05}$ 
        & $2.64{\scriptstyle\pm.07}$ \\
        & DenseNet100 
        & $0.56{\scriptstyle\pm.01}$ 
        & $1.24{\scriptstyle\pm.04}$ 
        & $2.56{\scriptstyle\pm.19}$ \\
      \bottomrule
      \end{tabular}}
    \label{T:xxx}
\end{table*}

==> tables/dataset.tex <==
\begin{table}[t]
    \centering
    \caption{Statistics of the computer vision datasets.}
    \begin{threeparttable}
      \begin{tabular}{lccc}
       \toprule
       {Datasets} & \# Samples & \# Classes & \# Dimensions \\
       \midrule
      CIFAR10 & 60,000 & 10 & $32\times32\times3$  \\
      CIFAR100 & 60,000 & 100 & $32\times32\times3$  \\
      \bottomrule
      \end{tabular}
    \end{threeparttable}
    \label{T:data-cv}
\end{table}


\begin{table}[t]
    \centering
    \caption{Statistics of the graph datasets.}
    \begin{threeparttable}
    \resizebox{1\columnwidth}{!}{
    \begin{tabular}{lcccc}
       \toprule
       {Datasets} & \# Nodes & \# Edges & \# Classes & \# Features \\
       \midrule
      Cora-ML & 2,995 & 16,346 & 7 & 2,879 \\
      CS & 18,333 & 163,788 & 15 & 6,805 \\
      Photos & 7,650 & 238,162 & 8 & 745 \\
      \bottomrule
      \end{tabular}
      }
    \end{threeparttable}
    \label{T:data-graph}
\end{table}

==> tables/graph-alpha-2.tex <==
\begin{table*}[t]
    \centering
    \caption{The efficiency results of conformal correction methods on graph datasets when $\alpha=0.2$. The results are the average of five runs of pre-trained model, each with 100 runs of conformal splits on graph datasets. 
    The best results are in shadow.}
    \setlength{\tabcolsep}{3.5mm}{
      \begin{tabular}{lccccccc}
      \toprule
      \multirow{2}{*}{Dataset} & \multirow{2}{*}{Model} & \multicolumn{2}{c}{CP} & \multicolumn{2}{c}{CF-GNN} & \multicolumn{2}{c}{CCN} \\
      \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}
       &  & Coverage & Efficiency & Coverage & Efficiency & Coverage & Efficiency \\
      \midrule
      \multirow{3}*{Cora-ML} 
       & GCN 
       & $0.80{\scriptstyle\pm.00}$
       & $3.10{\scriptstyle\pm.23}$ 
       & $0.80{\scriptstyle\pm.00}$  
       & $1.41{\scriptstyle\pm.10}$ 
       & $0.80{\scriptstyle\pm.00}$ 
       & \hl{$1.03{\scriptstyle\pm.03}$}  \\
       & GAT 
       & $0.80{\scriptstyle\pm.00}$ 
       & $3.07{\scriptstyle\pm.11}$  
       & $0.80{\scriptstyle\pm.00}$  
       & $1.47{\scriptstyle\pm.15}$  
       & $0.80{\scriptstyle\pm.00}$ 
       & \hl{$1.10{\scriptstyle\pm.06}$}  \\
         & SGC 
         & $0.80{\scriptstyle\pm.00}$ 
         & $3.11{\scriptstyle\pm.15}$  
         & $0.80{\scriptstyle\pm.00}$  
         & $1.42{\scriptstyle\pm.12}$  
         & $0.80{\scriptstyle\pm.00}$ 
         & \hl{$1.03{\scriptstyle\pm.04}$}  \\
        \midrule
       \multirow{3}*{CS}
       & GCN 
       & $0.80{\scriptstyle\pm.00}$ 
       & $6.12{\scriptstyle\pm.23}$  
       & $0.80{\scriptstyle\pm.00}$  
       & $2.66{\scriptstyle\pm.12}$  
       & $0.80{\scriptstyle\pm.00}$ 
       & \hl{$1.73{\scriptstyle\pm.14}$}  \\
         & GAT 
       & $0.80{\scriptstyle\pm.00}$ 
       & $5.18{\scriptstyle\pm.19}$  
       & $0.80{\scriptstyle\pm.00}$  
       & $3.24{\scriptstyle\pm.13}$  
       & $0.80{\scriptstyle\pm.00}$ 
       & \hl{$1.74{\scriptstyle\pm.17}$}  \\
       & SGC 
       & $0.80{\scriptstyle\pm.00}$ 
       & $6.15{\scriptstyle\pm.25}$  
       & $0.80{\scriptstyle\pm.00}$  
       & $3.24{\scriptstyle\pm.20}$  
       & $0.80{\scriptstyle\pm.00}$ 
       & \hl{$1.84{\scriptstyle\pm.15}$}  \\
        \midrule
        \multirow{3}*{Photos}
       & GCN 
       & $0.80{\scriptstyle\pm.00}$ 
       & $3.11{\scriptstyle\pm.14}$  
       & $0.80{\scriptstyle\pm.00}$  
       & $1.58{\scriptstyle\pm.31}$  
       & $0.80{\scriptstyle\pm.00}$ 
       & \hl{$1.24{\scriptstyle\pm.07}$}  \\
       & GAT 
       & $0.80{\scriptstyle\pm.00}$ 
       & $1.83{\scriptstyle\pm.19}$  
       & $0.80{\scriptstyle\pm.00}$  
       & $1.74{\scriptstyle\pm.47}$  
       & $0.80{\scriptstyle\pm.00}$ 
       & \hl{$1.61{\scriptstyle\pm.12}$}  \\
       & SGC       
       & $0.80{\scriptstyle\pm.00}$ 
       & $3.13{\scriptstyle\pm.05}$  
       & $0.80{\scriptstyle\pm.00}$  
       & $1.44{\scriptstyle\pm.28}$  
       & $0.80{\scriptstyle\pm.00}$ 
       & \hl{$1.35{\scriptstyle\pm.09}$}  \\
      \bottomrule
      \end{tabular}}
    \label{T:graph-alpha-2}
\end{table*}

==> tables/graph-entropy-1.tex <==
\begin{table*}[t]
    \centering
    \caption{The entropy results of conformal correction methods on graph datasets when $\alpha=0.1$. The results are the average of five runs of pre-trained model, each with 100 runs of conformal splits on graph datasets.}
    \setlength{\tabcolsep}{3.5mm}{
      \begin{tabular}{lcccc}
      \toprule
       {Dataset} & {Model} & {CP} & {CF-GNN} & {CCN} \\
      \midrule
      \multirow{3}*{Cora-ML} & GCN & $0.74{\scriptstyle\pm.28}$ & $2.12{\scriptstyle\pm.37}$ & $2.32{\scriptstyle\pm.01}$ \\
       & GAT  & $0.76{\scriptstyle\pm.11}$ & $2.29{\scriptstyle\pm.30}$ & $2.37{\scriptstyle\pm.02}$ \\
        & SGC & $0.76{\scriptstyle\pm.14}$ & $2.30{\scriptstyle\pm.16}$ & $2.33{\scriptstyle\pm.02}$ \\
        \midrule
       \multirow{3}*{CS} & GCN  & $0.40{\scriptstyle\pm.07}$ & $3.40{\scriptstyle\pm.10}$ & $3.00{\scriptstyle\pm.22}$ \\
        & GAT & $0.57{\scriptstyle\pm.11}$ & $3.39{\scriptstyle\pm.11}$ & $2.90{\scriptstyle\pm.27}$ \\
        & SGC & $0.49{\scriptstyle\pm.07}$ & $3.39{\scriptstyle\pm.08}$ & $2.93{\scriptstyle\pm.32}$ \\
        \midrule
        \multirow{3}*{Photos} & GCN  & $0.62{\scriptstyle\pm.04}$ & $2.28{\scriptstyle\pm.76}$ & $2.19{\scriptstyle\pm.03}$ \\
       & GAT  & $1.32{\scriptstyle\pm.18}$ & $2.33{\scriptstyle\pm.73}$ & $2.25{\scriptstyle\pm.04}$ \\
      & SGC & $0.66{\scriptstyle\pm.04}$ & $2.22{\scriptstyle\pm.84}$ & $2.13{\scriptstyle\pm.03}$ \\
      \bottomrule
      \end{tabular}}
    \label{T:xxx}
\end{table*}

==> tables/graph-entropy-2.tex <==
\begin{table*}[t]
    \centering
    \caption{The entropy results of conformal correction methods on graph datasets when $\alpha=0.2$. The results are the average of five runs of pre-trained model, each with 100 runs of conformal splits on graph datasets.}
    \setlength{\tabcolsep}{3.5mm}{
      \begin{tabular}{lcccc}
      \toprule
       {Dataset} & {Model} & {CP} & {CF-GNN} & {CCN} \\
      \midrule
      \multirow{3}*{Cora-ML} & GCN & $0.74{\scriptstyle\pm.28}$ & $2.34{\scriptstyle\pm.06}$ & $2.39{\scriptstyle\pm.18}$ \\
       & GAT  & $0.76{\scriptstyle\pm.11}$ & $2.39{\scriptstyle\pm.03}$ & $2.38{\scriptstyle\pm.13}$ \\
        & SGC  & $0.76{\scriptstyle\pm.14}$ & $2.35{\scriptstyle\pm.05}$ & $2.46{\scriptstyle\pm.20}$ \\
        \midrule
       \multirow{3}*{CS} & GCN  & $0.40{\scriptstyle\pm.07}$ & $2.97{\scriptstyle\pm.01}$ & $3.56{\scriptstyle\pm.08}$ \\
        & GAT & $0.57{\scriptstyle\pm.11}$ & $2.99{\scriptstyle\pm.01}$ & $3.56{\scriptstyle\pm.14}$ \\
       & SGC & $0.49{\scriptstyle\pm.07}$ & $2.96{\scriptstyle\pm.01}$ & $3.58{\scriptstyle\pm.07}$ \\
        \midrule
        \multirow{3}*{Photos} & GCN  & $0.62{\scriptstyle\pm.04}$ & $2.23{\scriptstyle\pm.75}$ & $2.20{\scriptstyle\pm.02}$ \\
       & GAT  & $1.32{\scriptstyle\pm.18}$ & $2.70{\scriptstyle\pm.46}$ & $2.25{\scriptstyle\pm.03}$ \\
      & SGC  & $0.66{\scriptstyle\pm.04}$ & $2.18{\scriptstyle\pm.84}$ & $2.12{\scriptstyle\pm.02}$ \\
      \bottomrule
      \end{tabular}}
    \label{T:xxx}
\end{table*}

==> tables/hyperparameter_basemodel.tex <==
\begin{table}[t]
    \centering
    \caption{Hyperparameters for base models.}
    \begin{threeparttable}
      \begin{tabular}{lccc}
       \toprule
       Domain & Model & Depth &  Dropout \\
       \midrule
      \bottomrule
      \end{tabular}
    \end{threeparttable}
    \label{}
\end{table}
